Fair Representation Learning with Controllable High Confidence Guarantees via Adversarial Inference

Representation learning is increasingly applied to generate representations that generalize well across multiple downstream tasks. Ensuring fairness guarantees in representation learning is crucial to prevent unfairness toward specific demographic groups in downstream tasks. In this work, we formally introduce the task of learning representations that achieve high-confidence fairness. We aim to guarantee that demographic disparity in every downstream prediction remains bounded by a *user-defined* error threshold $\epsilon$, with *controllable* high probability. To this end, we propose the ***F**air **R**epresentation learning with high-confidence **G**uarantees (FRG)* framework, which provides these high-confidence fairness guarantees by leveraging an optimized adversarial model. We empirically evaluate FRG on three real-world datasets, comparing its performance to six state-of-the-art fair representation learning methods. Our results demonstrate that FRG consistently bounds unfairness across a range of downstream models and tasks.

==> 07-conclusion.tex <==
% \vspace{-0.6cm}
\section{Conclusion}
% \vspace{-0.1cm}
In this work, we introduced \proj, an FRL framework that provides high-confidence fairness guarantees, ensuring that unfairness for all downstream models and tasks is upper-bounded by a user-defined threshold. 
% The framework has three major components. The candidate selection (Sec.~\ref{sec:cs}) the adversarial predictor (Sec.~\ref{sec:adv}) and the fairness test (Sec.~\ref{sec:ft}). 
After substantiating our work with theoretical analysis, we conducted empirical evaluations that demonstrate \proj's effectiveness in upper-bounding unfairness across various downstream models and tasks.
